Gradient-based shape optimization for the reduction of particle erosion in bended pipes

In this paper we consider a shape optimization problem for the minimization of the erosion, that is caused by the impact of inert particles onto the walls of a bended pipe. Using the continuous adjoint approach, we formally compute the shape derivative of the optimization problem, which is based on a one-way coupled, fully Eulerian description of a monodisperse particle jet, that is transported in a carrier fluid. We validate our approach by numerically optimizing a three-dimensional pipe segment with respect to a single particle species using a gradient descent method, and show, that the erosion rates on the optimized geometry are reduced with respect to the initial bend for a broader range of particle Stokes numbers.

==> ProofGradientComputation.tex <==
\begin{proof}
For the differentiation of $\dependence{\lagrangianSturmApproach}{\pertubedDomain,\ansatzSpaceSturmApproachLetterPertubed,\testSpaceSturmApproachLetterPertubed}$
 with $\ansatzSpaceSturmApproachLetterPertubed \in \spaceEDeformed$
 and $\testSpaceSturmApproachLetterPertubed \in \spaceFDeformed$
 we reparametrize 
 $\spaceEDeformed$ and $\spaceFDeformed$ by elements of $\spaceE$ and $\spaceF$  composed with $\inverse{\transformationFromReferenceDomain}$ and introduce
 \begin{equation*}
   \dependence{\lagrangianSturmApproachTransformed}{\domainPertubationLetter,\ansatzSpaceSturmApproachLetter,\testSpaceSturmApproachLetter} 
   := \dependence{\lagrangianSturmApproach}{\pertubedDomain,\ansatzSpaceSturmApproachLetter \circ \inverse{\transformationFromReferenceDomain},\testSpaceSturmApproachLetter \circ \inverse{\transformationFromReferenceDomain}}.
 \end{equation*}
 An application of the transformation rule mapping the integrals defined on 
$\pertubedDomain$ to $\domain$ together with  \cref{lem:PropertiesOfTransformationAndDifferentialOperators}
yields 
  \begin{align}
    \begin{split}
      \label{eq:TransformedLagrangian}
    \dependence{\lagrangianSturmApproachTransformed}{\domainPertubationLetter,\ansatzSpaceSturmApproachLetter,\testSpaceSturmApproachLetter} 
    &=   \IntegralSurfacePartDomainPlain{\dependence{\costFunctionalBoundaryFunction}{\testSpaceSturmApproachResidenceTime} \detTrafoBdryEvaluated}{\surfaceCompDomainOutflow} 
     + \constantRegularizationTwo \IntegralSurfacePartDomainPlain{\detTrafoBdryEvaluated}{\surfaceCompDomainDeformable} \\
    &+ \constantRegularizationOne \IntegralDomain{ (\invTranspJacTrafoEvaluated \, \gradient{\testSpaceSturmApproachVelocity}) : (\invTranspJacTrafoEvaluated \, \gradient{\testSpaceSturmApproachVelocity})\detTrafoEvaluated } \\
    &+ \IntegralDomain{\reciprocal{\reynoldsNumber} 
    (\leviCivita (\jacobian{\ansatzSpaceSturmApproachVelocity} \, \invTranspJacTrafoEvaluated)_{\indJ \indK} ) 
    (\leviCivita (\jacobian{\testSpaceSturmApproachVelocity} \,\invTranspJacTrafoEvaluated)_{\indJ \indK}) 
    \detTrafoEvaluated} \\
    & + \IntegralSurfacePartDomainPlain{\etaPorosityOutflow (\ansatzSpaceSturmApproachVelocity \cdot \outerNormal)(\testSpaceSturmApproachVelocity \cdot \outerNormal)\detTrafoBdryEvaluated}{\surfaceCompDomainOutflow} 
    +\IntegralSurfacePartDomainPlain{(\ansatzSpaceSturmApproachVelocity\cdot\outerNormal - \velocityFluidInflow)\testSpaceSturmApproachInflowCondition \detTrafoBdryEvaluated}{\surfaceCompDomainInflow} \\
    & -\IntegralDomain{ \ansatzSpaceSturmApproachPressure \trace{\jacobian{\testSpaceSturmApproachVelocity} \, \invJacTrafoEvaluated}\detTrafoEvaluated} +\IntegralDomain{\testSpaceSturmApproachPressure \trace{\jacobian{\ansatzSpaceSturmApproachVelocity} \,\invJacTrafoEvaluated}\detTrafoEvaluated} \\
    &+\IntegralDomain{
    \Big(
      \ansatzSpaceSturmApproachVelocity \cdot \invTranspJacTrafoEvaluated \cdot \gradient{\ansatzSpaceSturmApproachResidenceTime}\testSpaceSturmApproachResidenceTime 
      +\reciprocal{\pecletNumber}
      (\invTranspJacTrafoEvaluated \cdot \gradient{\ansatzSpaceSturmApproachResidenceTime}) \cdot (\invTranspJacTrafoEvaluated \cdot \gradient{\testSpaceSturmApproachResidenceTime})
    \Big)
    \detTrafoEvaluated}\\
& - \IntegralDomain{\dependence{\rhsTransportEq}{\ansatzSpaceSturmApproachVelocity}\testSpaceSturmApproachResidenceTime \detTrafoEvaluated}.
    \end{split}
  \end{align}
  
   Note that 
  \begin{equation}
  \label{eq:ConnectionCostFunctionalLagrangian}
  \dependence{\costFunctionalLetter}{\domainControlled} 
  = \dependence{\lagrangianSturmApproachTransformed}{\domainPertubationLetter,\solutionSturmApproachDomainTransformed,\testSpaceSturmApproachLetter}
  \quad \forall \, \testSpaceSturmApproachLetter \in \spaceF,
  \end{equation}
  where 
  $\solutionSturmApproachDomainTransformed := \transpose{(\transpose{(\solutionSturmApproachTransformedVelocityFluid)},\solutionSturmApproachTransformedPressure,\solutionSturmApproachTransformedResidenceTime)}$
  with 
  $\solutionSturmApproachTransformedVelocityFluid \cdot \outerNormal = \velocityFluidInflow$ on $\surfaceCompDomainInflow$
  solves the forward equations on the transformed domain after pull-back to the reference domain
  \begin{align}
  \begin{split}
  \label{eq:ForwardEquationsForFormalLagrangeApproachTransformed}
    &\IntegralDomain{\reciprocal{\reynoldsNumber} 
    (\leviCivita (\jacobian{\solutionSturmApproachTransformedVelocityFluid} \, \invTranspJacTrafoEvaluated)_{\indJ \indK}) 
    (\leviCivita (\jacobian{\testSpaceSturmApproachVelocity} \, \invTranspJacTrafoEvaluated)_{\indJ \indK}) 
    \detTrafoEvaluated} \\
    &+ \IntegralSurfacePartDomainPlain{\etaPorosityOutflow (\solutionSturmApproachTransformedVelocityFluid \cdot \outerNormal)(\testSpaceSturmApproachVelocity \cdot \outerNormal)\detTrafoBdryEvaluated}{\surfaceCompDomainOutflow} 
    -\IntegralDomain{\solutionSturmApproachTransformedPressure \trace{\jacobian{\testSpaceSturmApproachVelocity} \, 
    \invJacTrafoEvaluated}\detTrafoEvaluated} \\
    &+\IntegralDomain{ \testSpaceSturmApproachPressure \trace{\jacobian{\solutionSturmApproachTransformedVelocityFluid} \,\invJacTrafoEvaluated}\detTrafoEvaluated} \\
    &+\IntegralDomain{
    \Big(
      \solutionSturmApproachTransformedVelocityFluid \cdot \invTranspJacTrafoEvaluated \cdot \gradient{\solutionSturmApproachTransformedResidenceTime}\testSpaceSturmApproachResidenceTime +\reciprocal{\pecletNumber}
      (\invTranspJacTrafoEvaluated \cdot \gradient{\solutionSturmApproachTransformedResidenceTime}) \cdot (\invTranspJacTrafoEvaluated \cdot \gradient{\testSpaceSturmApproachResidenceTime})
    \Big)
    \detTrafoEvaluated}\\
    &= \IntegralDomain{\dependence{\rhsTransportEq}{\solutionSturmApproachTransformedVelocityFluid}\testSpaceSturmApproachResidenceTime \detTrafoEvaluated} \quad \forall \, \testSpaceSturmApproachLetter \in \spaceF .
  \end{split}
  \end{align}
 
  Due to the regularity of $\invTranspJacTrafoEvaluated$, $\detTrafoEvaluated$ and $\detTrafoBdryEvaluated$, 
  there exist bounds for 
  $\solutionSturmApproachDomainTransformed$
  in analogy to 
  \cref{eq:EstimateSolutionStokesEquationNonHomogenousDirichletConditionsInflow,eq:EstimateSolutionResidenceTimeEquation}.
  In order to apply \cref{thm:SturmDifferentiabilityTheorem} for the computation of the shape derivative,
  we now verify that $\lagrangianSturmApproachTransformed$ with $\spaceESturmTheorem=\spaceE$ and $\spaceFSturmTheorem=\spaceF$ satisfies assumptions (H0)-(H3).
  
  \paragraph*{Verification of (H0)}
  The integrals in \cref{eq:ForwardEquationsForFormalLagrangeApproachTransformed} continuously depend on $\invTranspJacTrafoEvaluated$, $\detTrafoEvaluated$ and $\detTrafoBdryEvaluated$ and converge to $\functionalA$, $\functionalB$, $\functionalC$ and $\functionalRHSResidenceTime$ from \cref{eq:FunctionalsForwardEquations} respectively for $\domainPertubationLetter \rightarrow 0$. 
  By continuity the inf-sup condition of $\functionalB$ and the ellipticity of $\functionalA$ and $\functionalC$ translate to the corresponding integrals in \cref{eq:ForwardEquationsForFormalLagrangeApproachTransformed} for $\domainPertubationLetter$ sufficiently small. Therefore \cref{eq:ForwardEquationsForFormalLagrangeApproachTransformed} possesses a unique solution $\solutionSetAnsatzSpaceSturmApproach = \{ \solutionSturmApproachDomainTransformed \}$,
  which verifies condition (H0)(i).


  Conditions (ii) and (iii) are satisfied due to the continuity of the functions 
  $\closedInterval{0}{1}\ni \convexCombinationLetter \mapsto 
		      \dependence{\lagrangianSturmApproachTransformed}{\domainPertubationLetter,\solutionSturmTheoremLetter 
			  + \convexCombinationLetter (\solutionSturmTheoremPertubed -\solutionSturmTheoremLetter),\testSpaceSturmApproachLetter }$
  and $\closedInterval{0}{1}\ni \convexCombinationLetter \mapsto 
		      \directionalDHilbertSpaces{\ansatzSpaceSturmApproachLetter}{\dependence{\lagrangianSturmApproachTransformed}{\domainPertubationLetter,\solutionSturmTheoremLetter 
			  + \convexCombinationLetter (\solutionSturmTheoremPertubed -\solutionSturmTheoremLetter),\testSpaceSturmApproachLetter }}{\ansatzSpaceSturmApproachLetter}$  
  and (iv) holds by the definition of the Lagrangian in \cref{eq:LagrangianFunction}.
  
   \paragraph*{Verification of (H1)}
  Condition (H1) is satisfied since $\invTranspJacTrafoEvaluated$, $\detTrafoEvaluated$ and $\detTrafoBdryEvaluated$ are continuously differentiable.


\paragraph*{Verification of (H2)}
  Defining the averaged solution 
%   \begin{align*}
$
\averagedSolutionSturm 
  := \solutionSturmApproachDomain 
  + \convexCombinationLetter (\solutionSturmApproachDomainTransformed-\solutionSturmApproachDomain)
$
%   \end{align*}
we consider the solution set $\{ \adjointSolutionSturmApproachDomainTransformed\}\subset \spaceE$ 
with   
$\adjointSolutionSturmApproachDomainTransformed
:=\transpose{(\transpose{(\adjointSolutionSturmApproachVelocityFluidTransformed)},\adjointSolutionSturmApproachPressureTransformed,\adjointSolutionSturmApproachResidenceTimeTransformed,\adjointSolutionSturmApproachPressureInflowConditionTransformed)}$
of the averaged adjoint equation  
  \begin{equation}
  \label{eq:AveragedAdjointEquationDefinition}
  \IntegralZeroToOne{\directionalDHilbertSpaces{\ansatzSpaceSturmApproachLetter}{\dependence{\lagrangianSturmApproachTransformed}{\domainPertubationLetter,\averagedSolutionSturm,\adjointSolutionSturmApproachDomainTransformed}}{\ansatzSpaceSturmApproachLetter}} 
  =0 
  \quad \forall \ansatzSpaceSturmApproachLetter \in \spaceE .
  \end{equation}

  Proceeding similar to \cref{sec:LagrangianAndAdjointEquations}, 
  we derive the averaged adjoint transport equation
  \begin{align}
  \begin{split}
  \label{eq:AvgAdjWeakTransportEquation}
     &\IntegralZeroToOne{\IntegralDomain{-(\averagedSolutionSturmVelocityFluid \cdot \gradient{\adjointSolutionSturmApproachResidenceTimeTransformed})\ansatzSpaceSturmApproachResidenceTime
		      -(\trace{\jacobian{\averagedSolutionSturmVelocityFluid} \, \invTranspJacTrafoEvaluated})\ansatzSpaceSturmApproachResidenceTime \adjointSolutionSturmApproachResidenceTimeTransformed
		    \detTrafoEvaluated}} \\
     & + \IntegralZeroToOne{\IntegralDomain{\reciprocal{\pecletNumber}(\invTranspJacTrafoEvaluated \cdot \gradient{\adjointSolutionSturmApproachResidenceTimeTransformed})\cdot (\invTranspJacTrafoEvaluated \cdot \gradient{\ansatzSpaceSturmApproachResidenceTime}) \detTrafoEvaluated}} \\
     & + \IntegralZeroToOne{\IntegralSurfacePartDomainPlain{(\averagedSolutionSturmVelocityFluid \cdot \outerNormal) \ansatzSpaceSturmApproachResidenceTime \adjointSolutionSturmApproachResidenceTimeTransformed \detTrafoBdryEvaluated}{\surfaceCompDomainOutflow} } \\
     &= -\IntegralZeroToOne{\IntegralSurfacePartDomainPlain{\dependence{\partialD{\costFunctionalBoundaryFunction}{\ansatzSpaceSturmApproachResidenceTime}}{\averagedSolutionSturmResidenceTime}\ansatzSpaceSturmApproachResidenceTime \detTrafoBdryEvaluated}{\surfaceCompDomainOutflow}}
     \quad \forall \ansatzSpaceSturmApproachResidenceTime \in \spaceR ,
  \end{split}
\end{align}
  as well as the averaged adjoint Stokes equation
  \begin{align}
  \begin{split}
     \label{eq:AvgAdjWeakStokesEquation}
    &\IntegralZeroToOne{\IntegralDomain{\reciprocal{\reynoldsNumber}  
      (\leviCivita (\jacobian{\ansatzSpaceSturmApproachVelocity} \, \invTranspJacTrafoEvaluated)_{\indJ \indK}) 
      (\leviCivita (\jacobian{\adjointSolutionSturmApproachVelocityFluidTransformed} \, \invTranspJacTrafoEvaluated)_{\indJ \indK}) 
      \detTrafoEvaluated}} \\
      & + \IntegralZeroToOne{\IntegralDomain{\adjointSolutionSturmApproachPressureTransformed \trace{\jacobian{\ansatzSpaceSturmApproachVelocity} \, \invJacTrafoEvaluated} \detTrafoEvaluated}} \\
      &+\IntegralZeroToOne{\IntegralSurfacePartDomainPlain{\etaPorosityOutflow (\ansatzSpaceSturmApproachVelocity \cdot \outerNormal) (\adjointSolutionSturmApproachVelocityFluidTransformed \cdot \outerNormal) \detTrafoBdryEvaluated}{\surfaceCompDomainOutflow}} 
      + \IntegralZeroToOne{
	    \IntegralSurfacePartDomainPlain{(\ansatzSpaceSturmApproachVelocity \cdot\outerNormal )\adjointSolutionSturmApproachPressureInflowCondition \detTrafoBdryEvaluated}{\surfaceCompDomainInflow}
	    }\\
      &=   \IntegralZeroToOne{
		\IntegralDomain{\ansatzSpaceSturmApproachVelocity \cdot 
		    \Big(
			(
			- \adjointSolutionSturmApproachResidenceTimeTransformed\,
			\invTranspJacTrafoEvaluated \cdot \gradient{\averagedSolutionSturmResidenceTime} 
			)
			+\dependence{\partialD{\rhsTransportEq}{\ansatzSpaceSturmApproachVelocity}}{\averagedSolutionSturmVelocityFluid}
			\adjointSolutionSturmApproachResidenceTimeTransformed
		    \Big)
		     \detTrafoEvaluated}
	    }\\
% 	   & + \IntegralZeroToOne{
% 		\IntegralDomain{
% 		    \averagedSolutionSturmResidenceTime \adjointSolutionSturmApproachResidenceTimeTransformed
% 		    \trace{\jacobian{\ansatzSpaceSturmApproachVelocity} \, \invJacTrafoEvaluated}
% 		    \detTrafoEvaluated
% 		}
% 	     } 
% 	     - \IntegralZeroToOne{
% 		  \IntegralSurfacePartDomainPlain{
% 		    (\ansatzSpaceSturmApproachVelocity \cdot \outerNormal)
% 		    \averagedSolutionSturmResidenceTime \adjointSolutionSturmApproachResidenceTimeTransformed
% 		    \detTrafoBdryEvaluated
% 		  }{\surfaceCompDomainOutflow}
% 		} \\
      & -\IntegralZeroToOne{\IntegralDomain{2\,\constantRegularizationOne (\invTranspJacTrafoEvaluated \, \gradient{\averagedSolutionSturmVelocityFluid}) : (\invTranspJacTrafoEvaluated \, \gradient{\ansatzSpaceSturmApproachVelocity})\detTrafoEvaluated }}
      \quad \forall \ansatzSpaceSturmApproachVelocity \in \spaceX ,
    \end{split}
    \end{align}
  with incompressibility condition
  \begin{equation}
%   \begin{split}
   \label{eq:AvgAdjWeakStokesIncompressibility}
    \IntegralZeroToOne{\IntegralDomain{-\ansatzSpaceSturmApproachPressure \trace{\jacobian{\adjointSolutionSturmApproachVelocityFluidTransformed} \, \invJacTrafoEvaluated} \detTrafoEvaluated}}
   =0
   \quad \forall \ansatzSpaceSturmApproachPressure \in \spaceM .
%      \end{split}
  \end{equation}
  Given $\domainPertubationLetter > 0$ sufficiently small, 
  \cref{eq:AveragedAdjointEquationDefinition} 
  is well-posed due to \cref{thm:AdjointProblem}
  and the continuity of 
  $\detTrafo$, $\detTrafoBdry$ and $\invTranspJacTrafo$
  at $\domainPertubationLetter=0$.

  \paragraph*{Verification of (H3)}
  We make sure this assumption holds by showing that there is a sequence 
  $(\adjointSolutionSturmApproachSequence)_{\indSequence \in \N}$
  with $\domainPertubationLetterSequence \searrow 0 $ as $\indSequence \rightarrow \infty$,
  where $\{\adjointSolutionSturmApproachSubsequence \} = \dependence{\averagedAdjointSolutionSetLetter}{\domainPertubationLetterSequence,\solutionSturmApproachSubsequence,\solutionSturmApproachDomain}$
  converges weakly in $\spaceF$ to $\adjointSolutionSturmApproachLetter$ and that 
  ${(\domainPertubationLetter,\testSpaceSturmApproachLetter)\mapsto \dependence{\partialD{\lagrangianSturmApproachTransformed}{\domainPertubationLetter}}{\domainPertubationLetter,\solutionSturmApproachDomain,\testSpaceSturmApproachLetter}}$
  is weakly sequentially continuous.

  The boundedness of the sequence 
  $(\norm{\solutionSturmApproachDomainTransformed}_{\spaceE})_{\domainPertubationLetter \ge 0}$
  guarantees the boundedness of the sequence 
  $(\norm{\adjointSolutionSturmApproachDomainTransformed}_{\spaceF})_{\domainPertubationLetter \ge 0}$
  for $\domainPertubationLetter$ sufficiently small.
  This can be seen by taking 
  $\ansatzSpaceSturmApproachResidenceTime = \adjointSolutionSturmApproachResidenceTimeTransformed$, 
  $\ansatzSpaceSturmApproachVelocity = \adjointSolutionSturmApproachVelocityFluidTransformed$ and
  $\ansatzSpaceSturmApproachPressure = \adjointSolutionSturmApproachPressureTransformed$
  in \cref{eq:AvgAdjWeakTransportEquation,eq:AvgAdjWeakStokesEquation,eq:AvgAdjWeakStokesIncompressibility} respectively
  and using the continuity of the integrals at $\domainPertubationLetter=0$.
  Due to the boundedness of the sequence of adjoint solutions 
  there exists a weakly converging subsequence $\adjointSolutionSturmApproachSubsequence$ with limit $\weakLimitOfAdjointSolutionSubsequence \in \spaceF$.
  The strong convergence 
  $\solutionSturmApproachDomainTransformed \rightarrow \solutionSturmApproachDomain$
  in $\spaceE$, which is proved in \cref{lem:ContinuityOfPertubedForwardSolutionSturmApproach},
  can be used to pass to the limit $\domainPertubationLetter \searrow 0$
  in 
\cref{eq:AvgAdjWeakTransportEquation,eq:AvgAdjWeakStokesEquation,eq:AvgAdjWeakStokesIncompressibility}
  and we obtain
  \begin{equation*}
   \adjointSolutionSturmApproachSubsequence \rightharpoonup \adjointSolutionSturmApproachDomain
   \textup{ for }  \indSequence \rightarrow \infty,
  \end{equation*}
  where $\adjointSolutionSturmApproachDomain \in \spaceF$ solves the adjoint problem \cref{eq:WeakAdjointProblem}. 
  The uniqueness of the limit yields $\weakLimitOfAdjointSolutionSubsequence = \adjointSolutionSturmApproachDomain$.

Since condition (H1) is satisfied, we can compute the partial derivative
  \begingroup
  \allowdisplaybreaks
  \begin{align*}
   &\dependence{\partialD{\lagrangianSturmApproachTransformed}{\domainPertubationLetter}}{\domainPertubationLetter,\ansatzSpaceSturmApproachLetter,\testSpaceSturmApproachLetter}\\
   &=
   \IntegralSurfacePartDomainPlain{\dependence{\costFunctionalBoundaryFunction}{\testSpaceSturmApproachResidenceTime} \detTrafoBdryPrimeEvaluated}{\surfaceCompDomainOutflow} 
    + \IntegralSurfacePartDomainPlain{\constantRegularizationTwo  \detTrafoBdryPrimeEvaluated}{\surfaceCompDomainDeformable}\\
   &+ \IntegralDomain{\constantRegularizationOne (\invTranspJacTrafoPrimeEvaluated \, \gradient{\ansatzSpaceSturmApproachVelocity}) : (\invTranspJacTrafoEvaluated \, \gradient{\ansatzSpaceSturmApproachVelocity})\detTrafoEvaluated } \\
   & 
	+\IntegralDomain{\constantRegularizationOne (\invTranspJacTrafoEvaluated \, \gradient{\ansatzSpaceSturmApproachVelocity}) : (\invTranspJacTrafoPrimeEvaluated \,\gradient{\ansatzSpaceSturmApproachVelocity})\detTrafoEvaluated } \\
    & 
	+\IntegralDomain{\constantRegularizationOne (\invTranspJacTrafoEvaluated \, \gradient{\ansatzSpaceSturmApproachVelocity}) : (\invTranspJacTrafoEvaluated \,\gradient{\ansatzSpaceSturmApproachVelocity})\detTrafoPrimeEvaluated} \\
      &+ \IntegralDomain{\reciprocal{\reynoldsNumber} 
    (\leviCivita (\jacobian{\ansatzSpaceSturmApproachVelocity} \, \invJacTrafoPrimeEvaluated)_{\indJ \indK}) 
    (\leviCivita (\jacobian{\testSpaceSturmApproachVelocity} \,
    \invJacTrafoEvaluated)_{\indJ \indK}) 
    \detTrafoEvaluated} \\  
          & + \IntegralDomain{\reciprocal{\reynoldsNumber} 
    (\leviCivita (\jacobian{\ansatzSpaceSturmApproachVelocity} \,
    \invJacTrafoEvaluated)_{\indJ \indK}) 
    (\leviCivita (\jacobian{\testSpaceSturmApproachVelocity} \, \invJacTrafoPrimeEvaluated)_{\indJ \indK}) 
    \detTrafoEvaluated} \\  
          & + \IntegralDomain{\reciprocal{\reynoldsNumber} 
    (\leviCivita (\jacobian{\ansatzSpaceSturmApproachVelocity} \,
    \invJacTrafoEvaluated)_{\indJ \indK}) 
    (\leviCivita (\jacobian{\testSpaceSturmApproachVelocity} \, \invJacTrafoEvaluated)_{\indJ \indK}) 
    \detTrafoPrimeEvaluated} \\  
    &+\IntegralSurfacePartDomainPlain{\etaPorosityOutflow (\ansatzSpaceSturmApproachVelocity \cdot \outerNormal)(\testSpaceSturmApproachVelocity \cdot \outerNormal)\detTrafoBdryPrimeEvaluated}{\surfaceCompDomainOutflow}
     + \IntegralSurfacePartDomainPlain{(\ansatzSpaceSturmApproachVelocity\cdot\outerNormal - \velocityFluidInflow)\testSpaceSturmApproachInflowCondition \detTrafoBdryPrimeEvaluated}{\surfaceCompDomainInflow} \\
    &+\IntegralDomain{- \ansatzSpaceSturmApproachPressure \trace{\jacobian{\testSpaceSturmApproachVelocity} \, \invJacTrafoPrimeEvaluated}\detTrafoEvaluated} 
     +\IntegralDomain{- \ansatzSpaceSturmApproachPressure \trace{\jacobian{\testSpaceSturmApproachVelocity} \, \invJacTrafoEvaluated}\detTrafoPrimeEvaluated} \\
    &+\IntegralDomain{\testSpaceSturmApproachPressure \trace{\jacobian{\ansatzSpaceSturmApproachVelocity} \, \invJacTrafoPrimeEvaluated}\detTrafoEvaluated} 
     +\IntegralDomain{\testSpaceSturmApproachPressure \trace{\jacobian{\ansatzSpaceSturmApproachVelocity} \, \invJacTrafoEvaluated}\detTrafoPrimeEvaluated} \\
    &+\IntegralDomain{\ansatzSpaceSturmApproachVelocity \cdot \invTranspJacTrafoPrimeEvaluated \cdot \gradient{\ansatzSpaceSturmApproachResidenceTime}\testSpaceSturmApproachResidenceTime \detTrafoEvaluated} 
     +\IntegralDomain{\ansatzSpaceSturmApproachVelocity \cdot \invTranspJacTrafoEvaluated \cdot \gradient{\ansatzSpaceSturmApproachResidenceTime}\testSpaceSturmApproachResidenceTime \detTrafoPrimeEvaluated} \\
    &+\IntegralDomain{\reciprocal{\pecletNumber}
    (\invTranspJacTrafoPrimeEvaluated \cdot \gradient{\ansatzSpaceSturmApproachResidenceTime}) \cdot (\invTranspJacTrafoEvaluated \cdot \gradient{\testSpaceSturmApproachResidenceTime}) \detTrafoEvaluated}\\
    &+\IntegralDomain{\reciprocal{\pecletNumber}
    (\invTranspJacTrafoEvaluated \cdot \gradient{\ansatzSpaceSturmApproachResidenceTime}) \cdot (\invTranspJacTrafoPrimeEvaluated \cdot \gradient{\testSpaceSturmApproachResidenceTime}) \detTrafoEvaluated}\\
    &+\IntegralDomain{\reciprocal{\pecletNumber}
    (\invTranspJacTrafoEvaluated \cdot \gradient{\ansatzSpaceSturmApproachResidenceTime}) \cdot (\invTranspJacTrafoEvaluated \cdot \gradient{\testSpaceSturmApproachResidenceTime}) \detTrafoPrimeEvaluated}
    -\IntegralDomain{\dependence{\rhsTransportEq}{\ansatzSpaceSturmApproachVelocity}\testSpaceSturmApproachResidenceTime \detTrafoPrimeEvaluated},
  \end{align*}%
  \endgroup
 from which we see that for fixed $\ansatzSpaceSturmApproachLetter \in \spaceE$ the mapping 
 ${(\domainPertubationLetter,\testSpaceSturmApproachLetter)\mapsto \dependence{\partialD{\lagrangianSturmApproachTransformed}{\domainPertubationLetter}}{\domainPertubationLetter,\ansatzSpaceSturmApproachLetter,\testSpaceSturmApproachLetter}}$
  is weakly sequentially continuous.
  Therefore (H3) is satisfied. 
  Due to \cref{eq:ConnectionCostFunctionalLagrangian} we obtain 
  \begin{equation}
    \label{eq:ShapeGradientFromLagrangianEvaluation}
     \denoteEulerianDerivativeFunctionalDomain{\costFunctionalLetter}{\boundaryVelocity}
     = \dependence{\partialD{\lagrangianSturmApproachTransformed}{\domainPertubationLetter}}{0,\solutionSturmApproachDomain,\adjointSolutionSturmApproachDomain}
  \end{equation}
  with the solutions $\solutionSturmApproachDomain \in \spaceE$ of the forward problem \cref{eq:WeakForwardPDESystem}
  and $\adjointSolutionSturmApproachDomain \in \spaceF$ of the adjoint problem \cref{eq:WeakAdjointProblem}.
  Since $\surfaceCompDomainInflow$ and $\surfaceCompDomainOutflow$ are kept fixed,
  the boundary integrals in \cref{eq:ShapeGradientFromLagrangianEvaluation} vanish.
  For the evaluation of the remaining volume integrals we take \cref{eq:DifferentiationOfTransformationQuantities} 
  from \cref{lem:PropertiesOfTransformationAndDifferentialOperators} 
  into account.
  \end{proof}

==> ShapeDerivativeOfCostFunctional.tex <==
In this section we derive the Eulerian semiderivative of the cost function by an application of the material derivative free Lagrange approach \cite{sturm2013lagrange}.
After introducing the associated Lagrangian and an investigation of the adjoint equations in \cref{sec:LagrangianAndAdjointEquations},
the subsequent \cref{sec:ComputingTheGradient} is devoted to the validation of the prerequisites for the application of \cref{thm:SturmDifferentiabilityTheorem}. 
To the best of our knowledge the continuous model \cref{eq:StationaryResidenceTimeAndBoundaryConditions} 
for the fluid residence time has not been considered as PDE constraint 
in gradient-based optimal shape design so far
and a result similar to \cref{thm:ShapeGradient}
has not yet been derived in the literature.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% Lagrangian and adjoint equations
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Lagrangian and adjoint equations}
\label{sec:LagrangianAndAdjointEquations}

Set $\spaceE:= \spaceX \times \spaceM \times \spaceRZero$
and
$\spaceF:= \spaceXZero \times \spaceM \times \spaceR \times \spaceB$.
For 
$\ansatzSpaceSturmApproachLetter:=(\transpose{\ansatzSpaceSturmApproachVelocity},\ansatzSpaceSturmApproachPressure,\ansatzSpaceSturmApproachResidenceTime) \in \spaceE$
and $\testSpaceSturmApproachLetter:=(\transpose{\testSpaceSturmApproachVelocity},\testSpaceSturmApproachPressure,\testSpaceSturmApproachResidenceTime,\testSpaceSturmApproachInflowCondition)\in \spaceF$ 
we define 
\begin{align*}
 \dependence{\functionalEq}{\domain,\ansatzSpaceSturmApproachLetter,\testSpaceSturmApproachLetter}
 :=& \dependence{\functionalA}{\domain, \ansatzSpaceSturmApproachVelocity,\testSpaceSturmApproachVelocity} 
 - \dependence{\functionalB}{\domain,\testSpaceSturmApproachVelocity,\ansatzSpaceSturmApproachPressure} 
    +\dependence{\functionalB}{\domain,\ansatzSpaceSturmApproachVelocity,\testSpaceSturmApproachPressure} \\ 
    &+ \dependence{\functionalInflowVelocityFluid}{\domain,\ansatzSpaceSturmApproachVelocity,\testSpaceSturmApproachInflowCondition} 
    + \dependence{\functionalC}{\domain,\ansatzSpaceSturmApproachVelocity,\ansatzSpaceSturmApproachResidenceTime,\testSpaceSturmApproachResidenceTime} 
    - \dependence{\functionalRHSResidenceTime}{\domain,\ansatzSpaceSturmApproachVelocity,\testSpaceSturmApproachResidenceTime}
\end{align*}
for the PDE constraint
using the definitions from \cref{sec:WellPosednessMathematicalModel}
and introduce the Lagrangian 
\begin{equation}
 \label{eq:LagrangianFunction}
 \dependence{\lagrangianSturmApproach}{\domain,\ansatzSpaceSturmApproachLetter,\testSpaceSturmApproachLetter}
 := \dependence{\costFunctionalLetter}{\domain,\ansatzSpaceSturmApproachResidenceTime,\ansatzSpaceSturmApproachVelocity}
   + \dependence{\functionalEq}{\domain,\ansatzSpaceSturmApproachLetter,\testSpaceSturmApproachLetter}
\end{equation}
associated with the optimization problem \cref{eq:OptimizationProblem}.

The adjoint state equations are obtained by differentiating \cref{eq:LagrangianFunction}
with respect to $\ansatzSpaceSturmApproachLetter$ at 
$\ansatzSpaceSturmApproachLetter = \solutionSturmApproachDomain := \transpose{(\transpose{\solutionSturmApproachVelocityFluid},\solutionSturmApproachPressure,\solutionSturmApproachResidenceTime)}$ 
and 
$\testSpaceSturmApproachLetter = \adjointSolutionSturmApproachDomain :=
\transpose{(\transpose{\adjointSolutionSturmApproachVelocityFluid},\adjointSolutionSturmApproachPressure,\adjointSolutionSturmApproachResidenceTime,\adjointSolutionSturmApproachPressureInflowCondition)}$
and solving
\begin{equation}
\label{eq:DefinitionOfAdjointEquation}
 \directionalDHilbertSpaces{\ansatzSpaceSturmApproachLetter}{\dependence{\lagrangianSturmApproach}{\domain,\solutionSturmApproachDomain,\adjointSolutionSturmApproachDomain}}{\ansatzSpaceSturmApproachLetter}
 = 0 \quad \forall \ansatzSpaceSturmApproachLetter \in \spaceE.
\end{equation}
We sort for the different parts of $\ansatzSpaceSturmApproachLetter$ in Equation \cref{eq:DefinitionOfAdjointEquation} 
and obtain the adjoint transport equation
\begin{align*}
 \begin{split}
  &\IntegralDomain{-(\solutionSturmApproachVelocityFluid \cdot \gradient{\adjointSolutionSturmApproachResidenceTime})\ansatzSpaceSturmApproachResidenceTime
		    +\reciprocal{\pecletNumber} \gradient{\adjointSolutionSturmApproachResidenceTime}\cdot\gradient{\ansatzSpaceSturmApproachResidenceTime}
		   }
      + \IntegralSurfacePartDomainPlain{(\solutionSturmApproachVelocityFluid \cdot \outerNormal)\adjointSolutionSturmApproachResidenceTime   \ansatzSpaceSturmApproachResidenceTime }{\surfaceCompDomainOutflow} \\
      &=-\IntegralSurfacePartDomainPlain{\dependence{\partialD{\costFunctionalBoundaryFunction}{\ansatzSpaceSturmApproachResidenceTime}}{\solutionSturmApproachResidenceTime}\ansatzSpaceSturmApproachResidenceTime}{\surfaceCompDomainOutflow}
      \quad \forall \ansatzSpaceSturmApproachResidenceTime \in \spaceRZero , 
 \end{split}
\end{align*}
as well as the adjoint Stokes equation
\begin{align*}
   \begin{split}      
  &\IntegralDomain{\reciprocal{\reynoldsNumber}  (\curl{\ansatzSpaceSturmApproachVelocity})\cdot (\curl{\adjointSolutionSturmApproachVelocityFluid})
  }    
   + \IntegralDomain{\adjointSolutionSturmApproachPressure \divergence{\ansatzSpaceSturmApproachVelocity}} \\
   &+\IntegralSurfacePartDomainPlain{\etaPorosityOutflow (\ansatzSpaceSturmApproachVelocity \cdot \outerNormal) (\adjointSolutionSturmApproachVelocityFluid \cdot \outerNormal)}{\surfaceCompDomainOutflow} 
	+\IntegralSurfacePartDomainPlain{(\ansatzSpaceSturmApproachVelocity \cdot \outerNormal)\, \adjointSolutionSturmApproachPressureInflowCondition}{\surfaceCompDomainInflow} \\
     &=   \IntegralDomain{\ansatzSpaceSturmApproachVelocity \cdot 
     (
     -\gradient{\solutionSturmApproachResidenceTime}
      \adjointSolutionSturmApproachResidenceTime
      +
	\dependence{\partialD{\rhsTransportEq}{\ansatzSpaceSturmApproachVelocity}}{\solutionSturmApproachVelocityFluid} \adjointSolutionSturmApproachResidenceTime 
	)} 
%       +\IntegralDomain{\solutionSturmApproachResidenceTime \adjointSolutionSturmApproachResidenceTime \divergence{\ansatzSpaceSturmApproachVelocity}} \\
      -2\,\constantRegularizationOne \IntegralDomain{\gradient{\solutionSturmApproachVelocityFluid}:\gradient{\ansatzSpaceSturmApproachVelocity}}
%   -\IntegralSurfacePartDomainPlain{(\ansatzSpaceSturmApproachVelocity\cdot\outerNormal)\solutionSturmApproachResidenceTime \adjointSolutionSturmApproachResidenceTime}{\surfaceCompDomainOutflow} 
%   +\IntegralSurfacePartDomainPlain{(\ansatzSpaceSturmApproachVelocity \cdot \outerNormal)\, \adjointSolutionSturmApproachPressureInflowCondition}{\surfaceCompDomainInflow}
   \quad \forall \ansatzSpaceSturmApproachVelocity \in \spaceX , 
     \end{split}
\end{align*} 
with incompressibility condition
\begin{equation*}
\IntegralDomain{\ansatzSpaceSturmApproachPressure \divergence{\adjointSolutionSturmApproachVelocityFluid}} = 0 \quad \forall \ansatzSpaceSturmApproachPressure \in \spaceM .
\end{equation*}



For the sake of brevity we introduce 
\begin{align*}
\dependence{\functionalD}{\domain,\solutionSturmApproachVelocityFluid,\adjointSolutionSturmApproachResidenceTime,\ansatzSpaceSturmApproachResidenceTime}
 =& \dependence{\functionalC}{\domain,-\solutionSturmApproachVelocityFluid,\adjointSolutionSturmApproachResidenceTime,\ansatzSpaceSturmApproachResidenceTime}
      + \IntegralSurfacePartDomainPlain{(\solutionSturmApproachVelocityFluid \cdot \outerNormal)\adjointSolutionSturmApproachResidenceTime   \ansatzSpaceSturmApproachResidenceTime }{\surfaceCompDomainOutflow}, \\
\dependence{\functionalRHSAdjointResidenceTime}{\domain,\solutionSturmApproachResidenceTime,\ansatzSpaceSturmApproachResidenceTime}
 =&\IntegralSurfacePartDomainPlain{
			 -\dependence{\partialD{\costFunctionalBoundaryFunction}{\ansatzSpaceSturmApproachResidenceTime}}{\solutionSturmApproachResidenceTime}\ansatzSpaceSturmApproachResidenceTime
			      }{\surfaceCompDomainOutflow}, \\
 \dependence{\functionalAdjointVelocityFluid}{\domain, \solutionSturmApproachVelocityFluid,\solutionSturmApproachResidenceTime,\adjointSolutionSturmApproachResidenceTime,\ansatzSpaceSturmApproachVelocity} 
 =& 
	\IntegralDomain{\ansatzSpaceSturmApproachVelocity \cdot 
     (-\gradient{\solutionSturmApproachResidenceTime} 
      \adjointSolutionSturmApproachResidenceTime 
      +
	\dependence{\partialD{\rhsTransportEq}{\ansatzSpaceSturmApproachVelocity}}{\solutionSturmApproachVelocityFluid} \adjointSolutionSturmApproachResidenceTime 
	)}
%       +\IntegralDomain{\solutionSturmApproachResidenceTime \adjointSolutionSturmApproachResidenceTime \divergence{\ansatzSpaceSturmApproachVelocity}} \\
%   &-\IntegralSurfacePartDomainPlain{(\ansatzSpaceSturmApproachVelocity\cdot\outerNormal)\solutionSturmApproachResidenceTime \adjointSolutionSturmApproachResidenceTime}{\surfaceCompDomainOutflow} 
  -2\,\constantRegularizationOne \IntegralDomain{\gradient{\solutionSturmApproachVelocityFluid}:\gradient{\ansatzSpaceSturmApproachVelocity}},
  \\
  \dependence{\functionalAdjointInflowVelocityFluid}{\domain,\ansatzSpaceSturmApproachVelocity,\adjointSolutionSturmApproachPressureInflowCondition}
  =& \IntegralSurfacePartDomainPlain{(\ansatzSpaceSturmApproachVelocity \cdot \outerNormal)\, \adjointSolutionSturmApproachPressureInflowCondition}{\surfaceCompDomainInflow},
\end{align*}
where the differentiability of the Moreau-regularization $\costFunctionalBoundaryFunction$ and the right hand side $\rhsTransportEq$ in the residence time equation have been used.
The operator $\functionalD$ describes the transport of the adjoint material age $\adjointSolutionSturmApproachResidenceTime$ along the negative fluid streamlines
and the right hand side $\functionalRHSAdjointResidenceTime$ accounts for the adjoint inflow conditions depending on the integrand $\costFunctionalBoundaryFunction$ of the cost function.
The right-hand side $\functionalAdjointVelocityFluid$ %for the adjoint Stokes equation 
sums up all terms that can be evaluated once the solution of \cref{eq:WeakForwardPDESystem} as well as $\adjointSolutionSturmApproachResidenceTime$ are given
and $\functionalAdjointInflowVelocityFluid$ stems from the differentiation of the weak form of the inflow condition.
Given these abbreviations the well-posedness of \cref{eq:DefinitionOfAdjointEquation} is addressed in 
\begin{theorem}
\label{thm:AdjointProblem}
 The problem 
% \begin{empheq}[left=\empheqlbrace]{align}
\begin{align}
\begin{split}
\label{eq:WeakAdjointProblem}
\textup{Given } \domain\in\shapesAdmissable 
\textup{ and } (\solutionSturmApproachVelocityFluid,\solutionSturmApproachPressure,\solutionSturmApproachResidenceTime) &\in \spaceE 
\textup{ solving \eqref{eq:WeakForwardPDESystem}} 
\textup{ seek } \\
 (\adjointSolutionSturmApproachVelocityFluid,\adjointSolutionSturmApproachPressure,\adjointSolutionSturmApproachResidenceTime,\adjointSolutionSturmApproachPressureInflowCondition)  &\in \spaceF
    \textup{ s.t.} \\
    \dependence{\functionalD}{\domain,\solutionSturmApproachVelocityFluid,\adjointSolutionSturmApproachResidenceTime,\ansatzSpaceSturmApproachResidenceTime}
 &= \dependence{\functionalRHSAdjointResidenceTime}{\domain,\solutionSturmApproachResidenceTime,\ansatzSpaceSturmApproachResidenceTime} 
 \qquad\quad\;\;\; \forall \ansatzSpaceSturmApproachResidenceTime \in \spaceRZero \\
 \dependence{\functionalA}{\domain,\adjointSolutionSturmApproachVelocityFluid,\ansatzSpaceSturmApproachVelocity} 
 + \dependence{\functionalB}{\domain,\ansatzSpaceSturmApproachVelocity,\adjointSolutionSturmApproachPressure}
 &=  \dependence{\functionalAdjointVelocityFluid}{\domain,\solutionSturmApproachVelocityFluid,\solutionSturmApproachResidenceTime,\adjointSolutionSturmApproachResidenceTime,\ansatzSpaceSturmApproachVelocity} 
 \quad \forall \ansatzSpaceSturmApproachVelocity \in \spaceX \\
 \dependence{\functionalB}{\domain,\adjointSolutionSturmApproachVelocityFluid,\ansatzSpaceSturmApproachPressure} 
 &= 0
  \qquad\qquad\qquad\qquad\;\;\; \forall \ansatzSpaceSturmApproachPressure \in \spaceM \\
  \dependence{\functionalAdjointInflowVelocityFluid}{\domain,\ansatzSpaceSturmApproachVelocity,\adjointSolutionSturmApproachPressureInflowCondition}
  &=0
  \qquad\qquad\qquad\qquad\;\;\; \forall \ansatzSpaceSturmApproachVelocity \in \spaceX 
 \end{split}
\end{align} 
% \end{empheq}
possesses a unique solution and the estimates
\begin{subequations}
\begin{align}
\label{eq:EstimateAdjointSolutionResidenceTimeEquation}
 \norm{\adjointSolutionSturmApproachResidenceTime}_{\HOneDomain}
 &\le c \norm{\dependence{\functionalRHSAdjointResidenceTime}{\domain,\solutionSturmApproachResidenceTime,\cdot}}_{\HOneDomain}, \\
 \label{eq:EstimateSolutionAdjointStokesEquation}
\norm{\adjointSolutionSturmApproachVelocityFluid}_{\HOneDomainVect} 
  + \normLTwoDomain{\adjointSolutionSturmApproachPressure}
  &\le c 
	  \norm{\dependence{\functionalAdjointVelocityFluid}{\domain,\solutionSturmApproachVelocityFluid,\solutionSturmApproachResidenceTime,\adjointSolutionSturmApproachResidenceTime,\cdot}}_{\weakDifferentiableUpToOrder{\domain}{-1}^3}
\end{align}
\end{subequations}
hold. 
\end{theorem}
\begin{proof}
The ellipticity of $\functionalD$ follows from  \cref{thm:WellPosednessWeakStokesAndResidenceTimeModel}
and therefore the standard estimates \cref{eq:EstimateAdjointSolutionResidenceTimeEquation,eq:EstimateSolutionAdjointStokesEquation} hold.

\end{proof}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% 
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Computation of the shape gradient}
\label{sec:ComputingTheGradient}

After introducing the adjoint equations in the previous section,
we now address the shape differentiability of the cost function following ideas from \cite{gangl2015shape, sturm2015minimax}.

\begin{theorem}
 \label{thm:ShapeGradient}
 The function $\costFunctionalLetter$ is shape differentiable and its shape derivative in direction $\boundaryVelocity$ is given by
 \begin{align}
  \begin{split}
 \label{eq:ExpressionShapeGradient}
  \denoteEulerianDerivativeFunctionalDomain{\costFunctionalLetter}{\boundaryVelocity}
  =&  -\IntegralDomain{
	    \reciprocal{\reynoldsNumber}(
	    (\leviCivita (\jacobian{\solutionSturmApproachVelocityFluid} \, \jacobian{\boundaryVelocity}))_{\indJ \indK}\, \euclideanBasisVector{\indI}) \cdot(\curl{\adjointSolutionSturmApproachVelocityFluid})
      } \\
      & -\IntegralDomain{
	   \reciprocal{\reynoldsNumber}(\curl{\solutionSturmApproachVelocityFluid})\cdot
	   (\leviCivita (\jacobian{\adjointSolutionSturmApproachVelocityFluid} \, \jacobian{\boundaryVelocity})_{\indJ \indK}\, \euclideanBasisVector{\indI})
      } \\
      & - \IntegralDomain{
		    \big(
      			\adjointSolutionSturmApproachPressure \, \trace{\jacobian{\solutionSturmApproachVelocityFluid} \, \jacobian{\boundaryVelocity}}
			-\solutionSturmApproachPressure \, \trace{\jacobian{\adjointSolutionSturmApproachVelocityFluid} \,\jacobian{\boundaryVelocity} }
		     \big)
		} \\
      & - \IntegralDomain{
				(\solutionSturmApproachVelocityFluid \cdot \transpose{\jacobian{\boundaryVelocity}}
				\cdot \gradient{\solutionSturmApproachResidenceTime})
				\adjointSolutionSturmApproachResidenceTime
				} \\
      & - \IntegralDomain{
		    \reciprocal{\pecletNumber} 
		    \big(
		    (\transpose{\jacobian{\boundaryVelocity}} \cdot \gradient{\solutionSturmApproachResidenceTime})\cdot \gradient{\adjointSolutionSturmApproachResidenceTime}
		    +(\transpose{\jacobian{\boundaryVelocity}}\cdot \gradient{\adjointSolutionSturmApproachResidenceTime})
		    \cdot \gradient{\solutionSturmApproachResidenceTime} 
		    \big)
	      } \\
      & +\IntegralDomain{
	      \big(
	      \reciprocal{\reynoldsNumber} (\curl{\solutionSturmApproachVelocityFluid}) \cdot (\curl{\adjointSolutionSturmApproachVelocityFluid})
	      - \solutionSturmApproachPressure (\divergence{\adjointSolutionSturmApproachVelocityFluid})
	      \big) (\divergence{\boundaryVelocity})
	      } \\
      & + \IntegralDomain{
			  \adjointSolutionSturmApproachPressure (\divergence{\solutionSturmApproachVelocityFluid}) (\divergence{\boundaryVelocity})
			  } \\
      & + \IntegralDomain{
		  \big(
		  \solutionSturmApproachVelocityFluid \cdot \gradient{\solutionSturmApproachResidenceTime} \,\adjointSolutionSturmApproachResidenceTime
		  +\reciprocal{\pecletNumber} \gradient{\solutionSturmApproachResidenceTime} \cdot \gradient{\adjointSolutionSturmApproachResidenceTime}
		  - \dependence{\rhsTransportEq}{\solutionSturmApproachVelocityFluid}\adjointSolutionSturmApproachResidenceTime
		  \big)
		  (\divergence{\boundaryVelocity})
		} \\
      & +\constantRegularizationOne \IntegralDomain{\big(\matrixQShapeGradient \,\gradient{\solutionSturmApproachVelocityFluid}\big) : \gradient{\solutionSturmApproachVelocityFluid} }
	+ \constantRegularizationTwo \IntegralSurfacePartDomainPlain{\tangentialDivergence{\boundaryVelocity}}{\surfaceCompDomainDeformable},
  \end{split}	      
 \end{align}
 where 
 $\matrixQShapeGradient:= (\divergence{\boundaryVelocity})\identityMatrix - \transpose{\jacobian{\boundaryVelocity}} - \jacobian{\boundaryVelocity}$, 
 $\euclideanBasisVector{\indI}\in \R^{3}$ denotes the $\indI$-th standard basis vector
%  $\matrixPShapeGradient:= (\divergence{\boundaryVelocity})\identityMatrix - \jacobian{\boundaryVelocity}$,
 and 
 $\solutionSturmApproachDomain\in\spaceX$ and $\adjointSolutionSturmApproachDomain \in \spaceF$ are the unique solutions of \eqref{eq:WeakForwardPDESystem} and \eqref{eq:WeakAdjointProblem} respectively.
 \end{theorem}

\input{ProofGradientComputation.tex}
  
  
  The next \cref{lem:ContinuityOfPertubedForwardSolutionSturmApproach}
  addresses the convergence in norms of the solutions of  \eqref{eq:ForwardEquationsForFormalLagrangeApproachTransformed}, 
  which is used to verify Assumption (H3) in Theorem \ref{thm:ShapeGradient}.
  A continuity result for the instationary incompressible Navier-Stokes equations with different boundary conditions has been derived in \cite{lindemann2012theoretical}.
  Since we consider a non-standard formulation of the stationary incompressible Stokes equations with an additional advection-diffusion-reaction equation \cref{eq:WeakForwardPDESystem} in this paper, 
  \cref{lem:ContinuityOfPertubedForwardSolutionSturmApproach} represents a new result.
  
    \begin{lemma}
 \label{lem:ContinuityOfPertubedForwardSolutionSturmApproach}
 The sequence of solutions $\{ \solutionSturmApproachDomainTransformed\}_{\domainPertubationLetter} \in \spaceE$ 
  of  \eqref{eq:ForwardEquationsForFormalLagrangeApproachTransformed} 
 converges to the solution $\solutionSturmApproachDomain \in \spaceE$ of problem \eqref{eq:WeakForwardPDESystem}
 in the sense of norms, i.e. it holds
 \begin{equation*}
 \lim_{\domainPertubationLetter \searrow 0} \norm{\solutionSturmApproachDomainTransformed-\solutionSturmApproachDomain}_{\spaceE}=0.
 \end{equation*}
\end{lemma}
  
  \input{ProofNormConvergenceForwardSolutions.tex}
  
